Exploiting Extensive-Form Structure in Empirical Game-Theoretic Analysis

Empirical game-theoretic analysis (EGTA) is a general framework for reasoning about complex games using agent-based simulation. Data from simulating select strategy profiles is employed to estimate a cogent and tractable game model approximating the underlying game. To date, EGTA methodology has focused on game models in normal form; though the simulations play out in sequential observations and decisions over time, the game model abstracts away this temporal structure. Richer models of \textit{extensive-form games} (EFGs) provide a means to capture temporal patterns in action and information, using tree representations. We propose \textit{tree-exploiting EGTA} (TE-EGTA), an approach to incorporate EFG models into EGTA\@. TE-EGTA constructs game models that express observations and temporal organization of activity, albeit at a coarser grain than the underlying agent-based simulation model. The idea is to exploit key structure while maintaining tractability. We establish theoretically and experimentally that exploiting even a little temporal structure can vastly reduce estimation error in strategy-profile payoffs compared to the normal-form model. Further, we explore the implications of EFG models for iterative approaches to EGTA, where strategy spaces are extended incrementally. Our experiments on several game instances demonstrate that TE-EGTA can also improve performance in the iterative setting, as measured by the quality of equilibrium approximation as the strategy spaces are expanded.

==> app_subroutines.tex <==
% \subsection{Omitted Subroutines from Algorithm~\ref{alg:coarsen}}\label{app:subroutines}
In this section, we provide pseudocodes for the two subroutines \textbf{CoarsenInfosets} and \textbf{CondenseBranching} of the \textbf{Coarsen} algorithm from Section~\ref{sec:abstraction}. 
\begin{algorithm}
\label{alg:sub1}
\renewcommand{\thealgorithm}{}
\small
\floatname{algorithm}{CoarsenInfosets}
\caption{Subroutine for coarsening input game G's infosets}
\begin{algorithmic}
\Require{Set $I_j(c)$ of infosets induced by each outcome $e \in X(c)$ for player $j$, set $Z$ of intersecting histories across $I_j(c)$, map $\rho: C' \rightarrow X$, input game $G$, $H'$}
\vspace{1em}
\State Create a new infoset $I'_j = \bigcup_{e \in \rho(c)} \{ he \hspace{0.2em} | \hspace{0.2em} h \in Z \}$ and add to $\mathcal{I}'_j$
% \State Create a new infoset $I'_j = \bigcup_{e \in X(c)} \{ he \hspace{0.2em} | \hspace{0.2em} h \in Z \}$ consisting of all the child nodes whose histories minus the chance events were part of the intersection $Z$; add to $\mathcal{I}'_j$
% \State Compute the Cartesian product of the action spaces available at each infoset in $I_j(c)$ to create a new action space $\Pi'_j(I'_j) = \bigotimes_{I \in I_j(c)} \Pi_j(I)$.
\State Compute the new action space $\Pi'_j(I'_j) = \bigotimes_{I \in I_j(c)} \Pi_j(I)$.
\For{$ha \in H'$}
\If{$a$ was part of an action space of $I_j(c)$}
\State Let $\Pi'_j(I'_j, a) = \{ x | x \in \Pi'_j(I'_j), a \in x \}$ %the set of $k$ new actions that contain $a$ somewhere in the tuple
\State Replace $ha$ with $hb$ for each action tuple $b \in \Pi'_j(I'_j, a)$
\State Assign $V'(hb) = V(ha)$
\EndIf
\EndFor
\State Delete each $e \in \rho(C')$ from every history in both the new infosets created and $H'$.
\State Remove all duplicate histories from both the infosets and $H'$.\\
\vspace{1em}
\Return New infosets and action spaces $\{ I'_j, \Pi'_j(I'_j) \}$, $H'$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\label{alg:sub2}
\renewcommand{\thealgorithm}{}
\small
\floatname{algorithm}{CondenseBranching}
\caption{Subroutine for reducing the branching factor induced by the newly coarsened action tuples}
\begin{algorithmic}
\Require{Set of infosets and action spaces $\{ I'_j, \Pi'_j(I'_j) \}$, final output set $\mathcal{I}'_j$}
\vspace{1em}
\State $A = \mathsf{copy}(\Pi'_j(I'_j))$
\For{$h \in I'_j$}
\State $g = \mathsf{copy}(h)$ and $\Pi'_j(\{ g \}) = \langle \rangle$
\For{$x \in A, a \in x$}
\State Add new infoset $\{ g \}$ to $\mathcal{I}'_j$ if $\{ g \} \notin \mathcal{I}'_j$
\State Add $x[:\mathsf{index}(a)]$ to the action space $\Pi'_j(\{ g \})$ if $a \notin \Pi'_j(\{ g \})$
\State $g = g \hspace{0.2em} x[:\mathsf{index}(a)]$
\State $V'(g) = j$
\EndFor
\EndFor\\
\vspace{1em}
\Return $\mathcal{I}'_j$, $\Pi'_j$
\end{algorithmic}
\end{algorithm}
